MiShape: 3D Shape Modelling of Mitochondria in Microscopy

Fluorescence microscopy is a quintessential tool for observing cells and understanding the underlying mechanisms of life-sustaining processes of all living organisms. The problem of extracting 3D shape of mitochondria from fluorescence microscopy images remains unsolved due to the complex and varied shapes expressed by mitochondria and the poor resolving capacity of these microscopes. We propose an approach to bridge this gap by learning a shape prior for mitochondria termed as MiShape, by leveraging high-resolution electron microscopy data. MiShape is a generative model learned using implicit representations of mitochondrial shapes. It provides a shape distribution that can be used to generate infinite realistic mitochondrial shapes. We demonstrate the representation power of MiShape and its utility for 3D shape reconstruction given a single 2D fluorescence image or a small 3D stack of 2D slices. We also showcase applications of our method by deriving simulated fluorescence microscope datasets that have realistic 3D ground truths for the problem of 2D segmentation and microscope-to-microscope transformation.

==> teasers/hybrid.tex <==
\begin{figure}[t]
  \centering
\includegraphics[width=\linewidth]{figures/Picture1a.png}
\caption{We present shape modeling solution for mitochondria. We train generative network for implict shape modeling using 3D EM images of mitochondria, which can then be used to simulate variety of paradigms in fluorescence microscopy for use with several interesting applications.}
   \label{fig:teaser}
\end{figure}
\begin{figure*}[t]
  \centering
% \includegraphics[width=0.75\linewidth]{figures/Picture1b_wide.png}
\includegraphics[width=\linewidth]{figures/Teaser2_v2.png}
   %\caption{Implicit shape representation presents several advantages over rasterized formats, and still supports both rasterized and mesh formats for flexibly introducing desired properties to fluorescence microscopy images.}
   \caption{\textbf{Problems with raster representation (left):} Challenges of extracting 3D shape from microscope images are illustrated. Discrete grid in EM images pose challenge in translation of shapes to fluorescence microscope due to different digital and optical resolution. \textbf{Benefits of implicit representation (right):} Implicit shape representation presents several advantages over raster formats, and still supports both raster and mesh formats for flexibly introducing desired properties to fluorescence microscopy images.}
   \label{fig:teaser2}
\end{figure*}

==> teasers/one_column_two_separatefigures.tex <==
\begin{figure}[t]
  \centering
\includegraphics[width=\linewidth]{figures/Picture1a.png}
\caption{Teaser}
   \label{fig:teaser}
\end{figure}
\begin{figure}[t]
  \centering
 \includegraphics[width=\linewidth]{figures/Picture1b.png}
   \caption{Teaser2}
   \label{fig:teaser2}
\end{figure}

==> teasers/one_column_two_subfigures.tex <==
\begin{figure}[t]
  \centering
\includegraphics[width=\linewidth]{figures/Picture1a.png}\\
    \hline
 \includegraphics[width=\linewidth]{figures/Picture1b.png}
   \caption{Teaser}
   \label{fig:teaser}
\end{figure}

==> teasers/original_abhi.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=0.9\linewidth]{figures/teaser.png}
   \caption{Teaser}
   \label{fig:teaser}
\end{figure}

==> teasers/two_columns_two_separatefigures.tex <==
\begin{figure*}[b]
  \centering
\includegraphics[width=\linewidth]{figures/Picture1a_wide.png}
\caption{Teaser}
   \label{fig:teaser}
\end{figure*}

\begin{figure*}[t]
  \centering
 \includegraphics[width=\linewidth]{figures/Picture1b_wide.png}
   \caption{Teaser2}
   \label{fig:teaser2}
\end{figure*}

==> teasers/two_columns_two_subfigures.tex <==
\begin{figure*}[t]
  \centering
\includegraphics[width=\linewidth]{figures/Picture1a_wide.png}\\
    \hline
 \includegraphics[width=\linewidth]{figures/Picture1b_wide.png}
   \caption{Teaser}
   \label{fig:teaser}
\end{figure*}
